We Have a Package for You! A Comprehensive Analysis of Package Hallucinations by Code Generating LLMs

The reliance of popular programming languages such as Python and JavaScript on centralized package repositories and open-source software, combined with the emergence of code-generating Large Language Models (LLMs), has created a new type of threat to the software supply chain: package hallucinations. These hallucinations, which arise from fact-conflicting errors when generating code using LLMs, represent a novel form of package confusion attack that poses a critical threat to the integrity of the software supply chain. This paper conducts a rigorous and comprehensive evaluation of package hallucinations across different programming languages, settings, and parameters, exploring how a diverse set of models and configurations affect the likelihood of generating erroneous package recommendations and identifying the root causes of this phenomenon. Using 16 popular LLMs for code generation and two unique prompt datasets, we generate 576,000 code samples in two programming languages that we analyze for package hallucinations. Our findings reveal that that the average percentage of hallucinated packages is at least 5.2% for commercial models and 21.7% for open-source models, including a staggering 205,474 unique examples of hallucinated package names, further underscoring the severity and pervasiveness of this threat. To overcome this problem, we implement several hallucination mitigation strategies and show that they are able to significantly reduce the number of package hallucinations while maintaining code quality. Our experiments and findings highlight package hallucinations as a persistent and systemic phenomenon while using state-of-the-art LLMs for code generation, and a significant challenge which deserves the research community's urgent attention.

==> conclusion.tex <==
\section{Conclusion}
\label{sub:conclusion}






In this paper, we systematically studied package hallucinations in code generated by various LLMs, focusing on both commercial and open-source models. Our comprehensive analysis revealed that approximately 19\% of generated packages are fictitious, posing a critical threat to software security through package confusion attacks. We identified key behavioral patterns and characterized hallucinated packages, proposing effective mitigation strategies. Our findings underscore the importance of addressing package hallucinations to enhance the reliability and security of AI-assisted software development.


==> system_messages.tex <==
\noindent\textbf{Code Generation Phase:}
\begin{itemize}
    \item System Message: ``You are a coding assistant that generates (Python|JavaScript) code. Provide only the code and add additional explanatory text only when absolutely necessary. If no code is required to answer the question, simply reply `None'''
    \item Prompt: LLM Generated prompts from \cref{sec:prompts} and Stack Overflow dataset.
\end{itemize}

\noindent \textbf{Package Generation Phase - Heuristic 1:}
\begin{itemize}
    \item System Message: ``You are a coding assistant that determines (Python|JavaScript) packages necessary to execute code. Respond with only a list of (Python|JavaScript) packages, separated by commas and no additional text or formatting. If there is no code provided, respond `None', otherwise the response must begin with the name of a (Python|JavaScript) package.''
    \item Prompt: ``Which (Python|JavaScript) packages are required to run this code: [Code sample generated from code generation phase]''
\end{itemize}

\noindent \textbf{Package Generation Phase - Heuristic 2:}
\begin{itemize}
    \item System Message: ``You are a coding assistant that recommends (Python|JavaScript) packages that would be helpful to solve given problems. Respond with only a list of (Python|JavaScript) packages, separated by commas and no additional text or formatting. The response must begin with the name of a (Python|JavaScript) package.''
    \item Prompt: ``Which (Python|JavaScript) packages would be useful in solving the following coding problem: [Original LLM generated prompt or Stack Overflow question]''
\end{itemize}

